Multiview Attenuation Estimation and Correction

Measuring attenuation coefficients is a fundamental problem that can be solved with diverse techniques such as X-ray or optical tomography and lidar. We propose a novel approach based on the observation of a sample from a few different angles. This principle can be used in existing devices such as lidar or various types of fluorescence microscopes. It is based on the resolution of a nonlinear inverse problem. We propose a specific computational approach to solve it and show the well-foundedness of the approach on simulated data. Some of the tools developed are of independent interest. In particular we propose an efficient method to correct attenuation defects, new robust solvers for the lidar equation as well as new efficient algorithms to compute the Lambert W function and the proximal operator of the logsumexp function in dimension 2.

==> proxlogsumexp.tex <==
\section{On the prox of logsumexp}

At one point, we need to compute the proximal operator of the logsumexp function in dimension 2. This is in fact a question of independent interest - especially in arbitrary dimension - since logsumexp is a well-spread $C^\infty$ approximation of the $l^\infty$-norm. Here, we focus on the numerical resolution of the problem. 

Let $a>0$ and define
\begin{equation}
 \phi(x_1,x_2)=a \log(\exp(x_1)+\exp(x_2)) + \frac{1}{2}(x_1-z_1)^2 + \frac{1}{2}(x_2-z_2)^2.
\end{equation}
We are looking for 
\begin{equation}
 (x_1^*,x_2^*)= \argmin_{(x_1,x_2)\in \R^2} \phi(x_1,x_2).
\end{equation}
This is exactly the prox of logsumexp in dimension $2$. 

The system of nonlinear equations we need to solve is:
\begin{equation}\label{eq:system}
\left\{\begin{array}{l}
a\frac{\exp(x_1)}{\exp(x_1)+\exp(x_2)} + x_1 - z_1 = 0 \\
 a\frac{\exp(x_2)}{\exp(x_1)+\exp(x_2)} + x_2 - z_2 = 0.
 \end{array}\right.
\end{equation}
Now comes Jonas' trick. Let $\lambda = \frac{\exp(x_1)}{\exp(x_1)+\exp(x_2)}$, then \eqref{eq:system} becomes:
\begin{equation}
\left\{\begin{array}{l}
a\lambda+ x_1 - z_1 = 0 \\
a(1-\lambda) + x_2 - z_2 = 0.
 \end{array}\right.
\end{equation}
Notice that $\frac{\exp(x_2)}{\exp(x_1)+\exp(x_2)}=1-\lambda$, therefore:
\begin{equation}
\frac{1-\lambda}{\lambda} = \exp(x_1-x_2) = \exp(z_2-z_1-a)\exp(2a\lambda).
\end{equation}

We are now facing the problem of finding the root of the following function:
\begin{equation}
 f(\lambda) = \exp(z_2-z_1-a)\exp(2a\lambda) + \frac{\lambda-1}{\lambda}.
\end{equation}
There are two important advantages for this approach. 
First, we have to solve a 1D problem instead of a 2D problem. 
More importantly, we constrain $x=z - a\delta$, where $\delta$ lives on the 2D simplex naturally.

Let us collect a few properties of function $f$. First, we have:
\begin{equation}
 f'(\lambda) = 2a\exp(z_2-z_1-a)\exp(2a\lambda) + \frac{1}{\lambda^2} > 0, \forall \lambda\in\R.
\end{equation}
Therefore, $f$ is the gradient of a \emph{convex} function. 
To apply the convergence results of Newton's algorithm, we will need to compute $f''$ as well:
\begin{equation}\label{eq:fp}
 f''(\lambda) = 4a^2 \exp(z_2-z_1-a)\exp(2a\lambda) - \frac{2}{\lambda^3}.
\end{equation}
Finally, we plot functions $f$ for $z_1=3$, $z_2=1$ and various values of $a$ in Fig. \ref{fig:f}.
As can be seen on this figure, we need a well chosen initial guess for $\lambda_0$ in a Newton method. For instance, if $\lambda_0=1$, the method is likely to converge for $a=4$ (redest curve), but it will do so very slowly. 
\begin{figure}
 \centering
 \includegraphics[width=0.35\textwidth]{images/Exemples_f-crop.pdf}
 \caption{Graphs of function $f$ for $a \in [0.25,128]$ with a dyadic scale.}\label{fig:f}
\end{figure}

\subsection{A variant of Kantorovich's theorem}

In this section we aim at proving convergence of Newton algorithm. Kantorovich obtained a famous convergence result for this method. In here, I will use the following variation due to Mysovskikh. 

\begin{theorem}
 Let $f:\R\to \R$ be a $C^2$ function on the interval $B=[x_0-r, x_0+r]$.
 Assume that:
 \begin{enumerate}
  \item[i)] $f'(x)\neq 0, \forall x\in B$,
  \item[ii)] $|1/f'(x)|\leq \beta, \forall x\in B$,
  \item[iii)] $|f''(x)|\leq K, \forall x\in B$,
  \item[iv)] $f(x_0)\leq \eta$,
  \item[v)] $h=K\beta^2\eta<2$,
  \item[vi)] $r\geq \beta \eta \sum_{n=0}^\infty (h/2)^{2^n-1} \geq \beta \eta (1 + h/2)$.
 \end{enumerate}
 Then $f$ has a root on $B$ and the sequence: $x_{k+1} = x_k - f(x_k)/f'(x_k)$ converges quadratically to $x^*$:
 \begin{equation}
  |x_k-x^*|\leq \frac{\beta \eta (h/2)^{2^k-1}}{1-(h/2)^{2^k}}.
 \end{equation}
\end{theorem}
This theorem is quite awful to apply! It still gives some insight on the method. 
An important remark is that, in our case, $f''$ is not bounded on $[0,1]$ and we therefore need to restrict to a ball around $\lambda^*$. 
Another remark is that if $z_1\geq z_2$, then $x_1^*\geq x_2^*$, therefore $\lambda^*\geq \frac{1}{2}$, hence we can focus on the interval $I=[\frac{1}{2},1]$, ensuring boundedness of $f''$. Unfortunately, this is not enough to ensure convergence for all possible values of $a,z_1,z_2$.
If $z_2\geq z_1$, then we should define $\lambda = \frac{\exp(x_2)}{\exp(x_1)+\exp(x_2)}$ instead. Below, we focus on the case $z_1\geq z_2$.

\subsection{On the initial guess}

The initial guess $\lambda_0$ is completely critical for the convergence of Newton's method. 
It is readily seen in Fig. \ref{fig:f}, that Newton's method will have difficulties to converge for the redish curves if the starting point is far away from $\lambda^*$.

To find a good initial guess, we recall that the logsumexp function is an approximation of the $l^\infty$-norm. 
Notice that:
\begin{align}
 (x_1^*,x_2^*)&= \argmin_{(x_1,x_2)\in \R^2} \phi(x_1,x_2)  \\
 &=\frac{1}{\sqrt{a}}\argmin_{(x_1',x_2')\in \R^2} LSE(\sqrt{a}x')+\frac{1}{2}\|x'-z'\|,
\end{align}
where $x'=\frac{x}{\sqrt{a}}$, $z'=\frac{z}{\sqrt{a}}$ and $LSE(x) = \log(\sum_{i=1}^n\exp(x_i))$.

Assume that $x_1 \geq \hdots  \geq x_i$, then it is easy to establish that:
\begin{equation}
\frac{LSE(\alpha x)}{\alpha} -\frac{\log(n)}{\alpha}  \leq \|x\|_\infty \leq  \frac{LSE(\alpha x)}{\alpha}.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        
\end{equation}
This observation motivates choosing $\lambda_0$ as the solution of the proximal operator of the $l^\infty$-norm. This choice is definitely the most stable (never takes more than 5 iterations to get machine precision for a wide range of parameters), suggesting global quadratic convergence. We just need to prove it now :).



% 
% \paragraph{Property i)}
% 
% This property is for free by \eqref{eq:fp}.
% 
% \paragraph{Property ii)}
% 
% The question is what is the minimal value of $\beta$ we can expect. 
% A rough upper-bound is obtained by restricting to the interval $I$:
% \begin{align*}
%  |f''(\lambda)|&\leq 4a^2 \exp(z_2-z_1+a)+16.
% \end{align*}
% This is bad when $z_2-z_1+a\gg 1$, and - indeed - the derivative of $f$ can be as large as wanted at the minimum by increasing $a$.
% 
% 
% 
% 
% \paragraph{Property iii)}
% 
% \paragraph{Property iv)}
% 
% \paragraph{Property v)}
% 
% \paragraph{Property vi)}
% 







